Does Negative Sampling Matter? A Review with Insights into its Theory and Applications

Negative sampling has swiftly risen to prominence as a focal point of research, with wide-ranging applications spanning machine learning, computer vision, natural language processing, data mining, and recommender systems. This growing interest raises several critical questions: Does negative sampling really matter? Is there a general framework that can incorporate all existing negative sampling methods? In what fields is it applied? Addressing these questions, we propose a general framework that leverages negative sampling. Delving into the history of negative sampling, we trace the development of negative sampling through five evolutionary paths. We dissect and categorize the strategies used to select negative sample candidates, detailing global, local, mini-batch, hop, and memory-based approaches. Our review categorizes current negative sampling methods into five types: static, hard, GAN-based, Auxiliary-based, and In-batch methods, providing a clear structure for understanding negative sampling. Beyond detailed categorization, we highlight the application of negative sampling in various areas, offering insights into its practical benefits. Finally, we briefly discuss open problems and future directions for negative sampling.

==> 2-candidates.tex <==
\section{Where to sample from? -- Candidates}\label{sec:candidates}
Negative sampling methods focus on designing negative sampling distributions, and sample a small subset from the negative candidate set to subsitute the entire negative samples for accelerating the training process. Thus, the selection of negative sample candidates also play a significant role in negative sampling. Here, we answer the first question where should we sample negative examples from? In terms of the composition of the negative sample candidates, we summarize their selection methods into the following five categories.
\begin{itemize}
    \item \textbf{Global Selection} is one of the most common methods for negative sample candidate selection, sampling directly negative examples from all unobserved ones. Typically, positive pairs for a particular anchor are sparse compared with large numbers of unobserved examples. Thus, global selection is very time-consuming, especially in large-scale and sparse datasets. For example, in hard negative sampling strategy coupled with global selection, the model needs to compute similiarity scores between the anchor and all unobserved examples. 
    

    \item \textbf{Local Selection} is a popular method to improve the efficiency of global selection, which usually select a part of unobserved examples as negative sample candidates. Such a selection method is widely used for hard negative mining where similarity computations are only performed for a small number of negative candidates. A small negative sample candidate set is generated by a fast random sampling strategy. 
    
    
    \item \textbf{Mini-batch Selection} is a more efficient way to improve local selection, which leverages other examples in the current mini-batch as negative sample candidates. Such a method does not require any additional sampling operations, significantly boosting sampling efficiency.
    
    
    \item \textbf{Hop Selection} is a novel selection method for graph-structured data, which selects $k$-hop neighbors as negative sample candidates. This method effectively takes advantage of the graph structure where the information propagation mechanism provides theoretical support. However, matrix operation for obtaining $k$-hop neighbors is impractical for web-scale datasets. Therefore, a path obtained from a random walk or DFS is often considered a negative sample candidate. 
    
    
    \item \textbf{Memory-based Selection} utilizes a memory bank or a cache as a pool to store negative sample candidates, in which negative examples can be directly sampled from this pool. Such a method needs extra storage space but saves time on candidate selection in each step. As a result of these properties, memory-based selection is generally applied in the case of requiring an amount of negative examples.      
    
\end{itemize}




The abovementioned five selection methods demonstrate different sources of negative sample candidates. We can adopt various selection methods according to different application scenarios and their own characteristics. Note that these selection methods can be integrated into negative sampling algorithms presented in Section~\ref{sec:algorithms}.  
% Here, we depict an overview of selection methods in Table~\ref{tab:ns_candidate}, comprising of application scope and properity (Pros and Cons). 














% In order to quickly retrieve items from large-scale recommender systems, the efficiency of negative sampling has attracted more and more attention. In two-tower neural network models, in-batch negatives     


% ~\cite{yi2019sampling} two-tower by using batch negatives, using the positive items
% in a mini batch as shared negatives for all queries in the same batch. A general recipe of training such two-tower models is to optimize loss functions calculated from
% in-batch negatives, which are items sampled from a random minibatch.

% ~\cite{yang2020mixed} mixed negative sampling 







==> 2-framework.tex <==
\section{Negative Sampling Framework}\label{sec:framework}
We summarize existing negative sampling strategies from various domains and provide a universal negative sampling framework that contains a positive sampler, a negative sampler, and a trainable encoder. The overall framework of negative sampling is illustrated in Figure ~\ref{fig: ns_framework}. The positive sampler is applied for generating positive training pairs. For example, positive pairs in recommendation are sampled explicitly from the observed user-item interactions, while these in contrastive learning are generated implicitly by data augmentations. Negative training pairs are sampled by different negative sampling strategies via a negative sampler. The abovementioned sampled pairs serve as training data and are fed into a trainable encoder. The trainable encoder varies by application domains, such as graph neural networks (GNNs)~\cite{kipf2016semi, velivckovic2017graph, hamilton2017inductive} in graph representation learning, ResNet~\cite{he2016deep} in unsupervised visual representation learning, BERT~\cite{devlin2018bert} and RoBERTa~\cite{liu2019roberta} in unsupervised sentence embedding learning, Skip-Gram~\cite{mikolov2013distributed} in word embedding, TransE~\cite{bordes2013translating} and TransH~\cite{wang2014knowledge} in knowledge graph embedding. 

In light of application domains, the objective function applied in negative sampling framework can be divided into four categories, including BPR loss, cross-entropy loss, hinge loss, and InfoNCE loss. In general, BPR loss is utilized for recommendation, which aims to learn a higher log-likelihood of positive pairs than negative ones. Cross-entropy loss is developed for word embedding and graph representation learning, and its purpose is to maximize the log-likelihood of positive pairs and minimize that of negative ones. Hinge loss is a common objective function for metric learning and knowledge graph embedding to estimate the discrepancy between negative pair and positive pair by a pre-set margin. Contrastive learning generally takes InfoNCE loss as objective optimization, which focuses on contrasting positive pairs and negative pairs. These abovementioned loss functions possess a unified keypoint of pulling positive pairs closer and pushing negative pairs away in the latent representation space. The specific formulations of these functions are presented in Figure~\ref{fig: ns_framework}.





% \begin{table}[thb]
% \centering
% \caption{An overview of loss functions in negative sampling framework.}
% \renewcommand{\arraystretch}{1.5}
% \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{c|c}  
% \hline
% \multirow{5}{*}{}   Type   &  Formulation   \\
% \hline
% BPR  &  $\mathcal{L} = \text{In}\sigma( \!z_u \cdot \!z_v^{-} - \!z_u \cdot \!z_v^{+})$ \\
% Cross-entropy  & $\mathcal{L} = - [\log\sigma(\!z_u \cdot \!z_v^{+}) + \log(\sigma(-\!z_u \cdot \!z_v^{-}))]$ \\
% Hinge  & $\mathcal{L} = \text{max}(0, \!z_u \cdot \!z_v^{-} - \!z_u \cdot \!z_v^{+}+\gamma) $ \\
% InfoNCE  & $\mathcal{L} = -\log \frac{e^{f(x)^Tf(x^+)}}{e^{f(x)^Tf(x^+)} + \sum_{k=1}^{K} e^{f(x)^Tf(x_k^-)} } $ \\
%     \hline
%     \end{tabular}}
% \label{tab:ns_loss}
% \end{table}


Here, we also present two popular learning methods: metric learning and contrastive learning. Such methods measure or compare the agreement and disconsistency between positive and negative pairs. 



\noindent \textbf{Negative Sampling in Metric Learning.}
The goal of metric learning is to automatically develop a metric from data that can be used to assess the similarity or distance between positive and negative pairs. The formulation of metric learning can be represented as follows: 
\begin{equation*}
    L=max(D(f(a), f(p)) - D(f(a), f(n)) + \alpha, 0)
\end{equation*}
where $(a, p)$ denotes a positive pair, $(a, n)$ is a sampled negative pair, and $D(\cdot)$ represents a distance measure function. The model $f$ is formalized for a triple loss optimization. Negative sampling plays a significant role in the success of metric learning where informative negative samples can provide useful gradients and speed up the training process. 



\noindent \textbf{Negative Sampling in Contrastive Learning.}
Contrastive learning is a dominant approach in self-supervised learning, showing tremendous potential in unsupervised learning (e.g. computer vision, natural language processing, and graph representation learning). The goal of contrastive learning is to pull a positive pair close to each other and push negative pairs apart in the embedding space through contrastive loss (See Figure~\ref{fig: ns_contrastive}). The InfoNCE loss is the most prominent contrastive loss derived from CPC~\cite{oord2018representation}, designed to maximize the similarity between positive pairs while simultaneously minimizing the similarity between negative pairs. It contrasts a positive pair $(z_i, z_j)$ generated by the data augmentations from $K$ negative pairs, which can be represented as follows:
\begin{equation*}
    L=-\log\frac{exp(sim(z_i,z_j)/\tau)}{exp(sim(z_i,z_j)/\tau) + \sum_{k=1}^{K}exp(sim(z_i, z_k)/\tau)}
\end{equation*}
where $sim(\cdot)$ is a cosine function to measure the similarity between two embeddings.
\begin{figure}[bthp]
  \centering
  \includegraphics[width=0.46\textwidth]{figures/ns_contrastive.pdf}
  \caption{Basic idea behind contrastive learning. }  
  \label{fig: ns_contrastive}
\end{figure}


==> 2-preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}
In this section, we introduce the preliminaries for various domains that employ negative sampling, consisting of settings (tasks, datasets, evaluation metrics) and basic encoders. 



\subsection{Recommendation}
Recommendation is the most important technique for information filtering in many E-commerce platforms, which aims to recommend the most relevant $N$ items for a particular user based on the learned user and item embeddings. The mainstream recommendation models include traditional matrix factorization (e.g. BPR~\cite{rendle2012bpr}), neural network-based methods (e.g. NCF~\cite{he2017neural}), and graph neural network-based methods (e.g. PinSage~\cite{ying2018graph}, NGCF~\cite{wang2019neural}, and LightGCN~\cite{he2020lightgcn}). Recently, pairwise loss with negative sampling has become a dominant technique for recommendation. The BPR loss is the most common pairwise loss used for learning user and item embeddings by assigning a higher preference for observed user-item pair (positive pair) than unobserved one (negative pair). \textit{Movielens-1m, Yelp2018, Amazon, Alibaba, and Pinterest} are popularly used datasets. \textit{Top-$N$ recommendation} is a classical task for recommendation where $recall@N$ and $NDCG@N$ serve as evaluation methodologies.

% . In Top-$N$ recommendation, the recommended item list for a user is generated by ranking all items that are not interacted with by the user. Here, $recall@N$ and $NDCG@N$ serve as evaluation methodologies for Top-$N$ recommendation. 



\subsection{Graph Representation Learning}
Graph representation learning aims to transform nodes in the graph into low-dimensional node embedding, whose representative algorithms contain traditional Network Embedding models (e.g. DeepWalk~\cite{perozzi2014deepwalk}, LINE~\cite{tang2015line}, and node2vec~\cite{grover2016node2vec}) and Graph Neural Networks (e.g. GCN~\cite{kipf2016semi}, GraphSAGE~\cite{hamilton2017inductive} and GAT~\cite{velivckovic2017graph}). Such learned node embeddings facilitate a lot of downstream tasks, such as \textit{node classification and link prediction}. For the unsupervised setting, cross-entropy loss with negative sampling has become the mainstream embedding learning method, whose goal is to maximize the log-likelihood of positive pairs and minimize that of negative ones. For the node classification task, the commonly used datasets contain \textit{BlogCatalog, Wikipedia, PPI, DBLP, and Flickr}, where \textit{Micro-F1 and Macro-F1} act as evaluation metrics. \textit{Arxiv, Facebook, and PPI} are popularly used datasets in the link prediction task where \textit{AUC} is the standard evaluation metric. 





\subsection{Knowledge Graph Embedding}
Knowledge graph embedding aims to project entities and relations (e.g. triples $<h,r,t>$) in the knowledge graph into low-dimensional embeddings. The two mainstream types of knowledge graph embedding models contain translational distance-based methods (e.g. TransE~\cite{bordes2013translating}, TransH~\cite{wang2014knowledge}, TransR~\cite{lin2015learning}, TransD~\cite{ji2015knowledge}, and TransG~\cite{xiao2015transg}) and the semantic matching-based methods (e.g. RESCAL~\cite{nickel2011three}, DistMult~\cite{yang2014embedding}, and ComplEx~\cite{trouillon2016complex}). \textit{Link Prediction, Knowledge graph completion, question answering, and recommendation} are major downstream tasks for knowledge graph embedding. Margin-based ranking loss (e.g. hinge loss) is commonly used in knowledge graph embedding learning, which adopts negative sampling to generate negative triples. Here, \textit{FB15k-237, WN18 and WN18RR} are three common datasets in which \textit{mean reciprocal ranking (MRR), and hits@10} are applied to evaluate the performance. 






\subsection{Natural Language Processing}
In natural language processing, word embedding and sentence embedding are two of the most important tasks. The goal of word embedding is to build distributed representations of words in a vector space. Word2vec~\cite{mikolov2013distributed} is one of the most popular word embedding models where \textit{Skip-gram with Negative Sampling (SGNS)} is a significant training mode. \textit{Wikipedia} is a real-world corpus to train the Skip-gram model. There are two common tasks used to evaluate downstream performance in the word embedding domain: \textit{word analogy and word similarity}. For the word similarity task, \textit{SIMLEX-999, RW, WS353, MURK, WS353S, WS353R, and RG656} are evaluation datasets and \textit{the Spearman’s rank correlation coefficient} is used to measure the similarities between words. As for the word analogy task, \textit{accuracy} serves as the evaluation metric. Learning universal sentence embeddings is another fundamental task where \textit{BERT~\cite{devlin2018bert} and RoBERTa~\cite{liu2019roberta}} act as backbones. For unsupervised settings, negative sentences sampled from Wikipedia are used for objective optimization. The standard semantic textual similarity (STS) tasks are utilized to evaluate performance. 




\subsection{Computer Vision}
Unsupervised visual representation learning has become a significant learning method for downstream tasks in computer vision. Contrastive learning with negative sampling is a mainstream technique for visual representation learning where ResNet~\cite{he2016deep} acts as the backbone for learning image embeddings. 
By using the learned image embeddings, we later perform \textit{image classification task} with a linear classifier, where the \textit{Top-1 Accuracy and Top-5 Accuracy} are treated as evaluation metrics. \textit{CIFAR10, CIFAR100, STL10, and ImageNet} are commonly used datasets.






























% \noindent \textbf{Dataset.} Negative sampling methods face the data challenge since different datasets possess various properties. Besides, datasets are used differently with various downstream tasks and evaluation metrics, which also affect the effectiveness of negative sampling. Each domain has its own unique datasets and data processing, and we thus present some commonly used dataset for various domains. 




% \begin{table*}[hbt]
% \centering
% \caption{Statistics of the tasks and datasets.}
% \label{dataset}
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{c|c|c|c|c}  
% \hline
% \multirow{5}{*}{}   Domain & Algorithms & Tasks    & Datasets & Evaluation Metrics \\
% \hline
% \multirow{3}{*}{Recommendation}
%         & MovieLens & 2,625   &  100,000   & / \\
%         & Amazon    & 255,404 &  1,689,188 & / \\
%         & Alibaba  & 159,633 &  907,470   & / \\  
% \hline
% \multirow{1}{*}{Graph Representation Learning}
%         & Arxiv & 5,242 & 28,980 & /\\
% \hline
% \multirow{1}{*}{Knowledge Graph Embedding}
%         & BlogCatalog & 10,312 & 333,983& 39  \\
%     \hline
%     \end{tabular}}
% \end{table*}
